Declarative Smart Contracts

This paper presents DeCon, a declarative programming language for implementing smart contracts and specifying contract-level properties. Driven by the observation that smart contract operations and contract-level properties can be naturally expressed as relational constraints, DeCon models each smart contract as a set of relational tables that store transaction records. This relational representation of smart contracts enables convenient specification of contract properties, facilitates run-time monitoring of potential property violations, and brings clarity to contract debugging via data provenance. Specifically, a DeCon program consists of a set of declarative rules and violation query rules over the relational representation, describing the smart contract implementation and contract-level properties, respectively. We have developed a tool that can compile DeCon programs into executable Solidity programs, with instrumentation for run-time property monitoring. Our case studies demonstrate that DeCon can implement realistic smart contracts such as ERC20 and ERC721 digital tokens. Our evaluation results reveal the marginal overhead of DeCon compared to the open-source reference implementation, incurring 14% median gas overhead for execution, and another 16% median gas overhead for run-time verification.

==> property-spec.tex <==
% \subsection{Property specification}
% 
% \proto also uses Datalog to express safety properties
% as a database integrity constraint.
% Such constraints are monitored at run-time against concrete inputs.
% 
% Specifically, safety properties are specified as declarative queries
% on transaction histories and contract views. 
% These queries are specified in a bug query way, such that
% an nonempty derivation of such queries implies the violation of properties.
% For example, in ERC20 contract, the property that all
% account balance should add up to the contract's balance 
% can be specified as follows:
% \begin{equation}
%     q1() :- s = sum\;m: balanceOf(_,m), totalSuply(t), s!=t.
% \end{equation}
% And \proto will monitor the query result $q1$ during run-time,
% and reports a property violation when $q1$ is derived nonempty.
% 
% To enable expressing more complex properties, 
% some special relations are reserved:
% \begin{itemize}
%     \item $[view]'$ represents the view that is going to be updated 
%     by the current transaction. 
%     \item $function$ stores the name of the current transaction.
% \end{itemize}
% These two kinds of reserved relations can be used to specify 
% properties that concern about inter-transaction changes.
% For example, in ERC20 contract, a property could state that 
% only $mint$ or $burn$ function can change the value of $totalSupply$:
% \begin{datalog}
% q2(f) :- totalSuply(s1), totalSuply'(s2),
%         s1 != s2, function(f), f != mint, f != burn.
% \end{datalog}


% \proto uses past time linear temporal logic to specify safety 
% properties, which have been shown to be able to express 
% a wide range of contract-level properties in prior research~\cite{}.
% 
% The temporal operators:
% \begin{itemize}
%     \item $\square$ always.
%     \item $\blacklozenge$ once.
% \end{itemize}
% 
% In addition to contract states and views,
% we introduce three special constructs that support richer properties:
% \begin{itemize}
% \item Aggregate of the state variables, in the same notation as in
% the datalog rules.
% \item Variable values before the last transaction commit.
% \item A reserved variable $tx$ that stores the name of 
% the invoked transaction.
% \end{itemize}
% Properties that reason about the transaction name and state changes
% have been shown popular in prior smart contract verification 
% research~cite{}.
% 
% Propositional formula $\phi$ is inductively defined as:
% \begin{equation}
% \begin{aligned}
% \phi := & v \; binop \; v \\
%     & | \phi \land \phi | \phi \lor \phi 
%     | \neg \phi | \phi \implies \phi \\
% v := & Variable | Variable' \\
%      & | Function | Constant | sum(Variable) \\
% binop := & > | < | >= | <= | == \\
% \end{aligned}
% \end{equation}


==> sec_acknowledgements.tex <==
\section*{Acknowledgements}
We thank the anonymous reviewers of FSE'22 for their insightful
feedback and suggestions.
This work is supported by NSF CNS-2104882, NSF CNS-2107147, NSERC Discovery Grant, 
and Office of Naval Research grant on Security for resource limited 
networked Cyber-physical systems.



==> sec_verification.tex <==
\section{Run-time verification}\label{sec:verif}

\subsection{Specifying common vulnerabilities in datalog}
We identify a list of auxiliary relations that are 
useful for specifying common vulnerabilities in
smart contracts.

\textbf{Integer overflow}.
Integer overflow for addition happens if the sign of the
two operands are the same, and the sign of the sum
is opposite to the operands. 
Similarly, other arithmetic operations can be 
formally specified in the following rules:
\begin{datalog}
overflow(c,a,b) :- c=a+b, c<0, a>0, b>0.
overflow(c,a,b) :- c=a+b, c>0, a<0, b<0.
overflow(c,a,b) :- c=a*b, b != c/a.
overflow(c,a,b) :- c=a/b, b==0.
\end{datalog}

\textbf{Re-entrancy attacks}.
To monitor re-entrancy attack, we need predicates
that stores the pending transactions, i.e., 
transactions that have been called by not yet
committed or aborted.
Relation $pending(caller, tx, t, [p,...])$ means
$caller$ calls transaction named $tx$ at time $t$ with 
parameters $[p,...]$, and the transaction is currently
pending.
The re-entrancy attack can be specified in the
following rule:
\begin{datalog}
reentrancy(caller,tx) :- pending(caller, tx, t1, _),
                        pending(caller,tx,t2,_), t1!=t2.
\end{datalog}

\textbf{Transaction order dependency}.
To monitor transaction order dependency,
we need predicate that stores the reading and writing
access of each transaction.
$read(tx,b,v)$ and $write(tx,b,v)$ 
represents transaction $tx$, 
to be recorded on block $b$,
reads / writes to state variable $v$.
\begin{datalog}
tod(tx1,tx2,v) :- read(tx1,b,v), write(tx2,b,v),tx1!=tx2.
\end{datalog}
An optimization is that, since this transaction order
dependency only happens between transactions within
the same block, at run-time the system only needs
to store read write histories of the latest block.

\textbf{Locked Ether}.
We focus on monitoring one of the causes for 
locked ether, which is when the smart contract
relies on an external function that does not exist.
Predicate $exists(a)$ means address $a$ exists.
This information can be obtained from Solidity's 
built-in function [].
\begin{datalog}
locked_ehter(f,a) :- external_call(f,a), !exists(a).
\end{datalog}

\textbf{Unhandled exceptions}.
\proto generates Solidity codes such that all function
call's return value will be checked.

Given these specifications, 
in the form of datalog queries,
\proto performs run-time 
verification by generating instrumentation to the source
code that monitor the query outputs.
When any query output is derived, \proto
throw an exception, aborts the transaction,
and returns the query derivation result
for the property violation properties.

\subsection{Contract-specific properties}

\subsection{Generating instrumentation}

For each transaction, specified by a transaction commit rule,
\proto performs the following:
\begin{enumerate}
    \item Derive auxiliary facts.
    \item For every specified properties, if the transaction
    rule contains or derives relevant predicates, 
    add in instrumentation codes that check the corresponding 
    property.
\end{enumerate}

\proto has a list of built-in fact deriving rules
that derive auxiliary facts from transaction rules.

For example, whenever a transaction uses a arithmetic
addition operation, the corresponding facts $c=a+b$
is derived.
We then generate instrumentation to check the rest of
the rule condition in the transaction handling function.


Rules to derive pending transactions.
\begin{datalog}
new pending(caller, tx_name, [p,...]) :- call_tx(caller, tx_name, [p,...]), 
                            now(time).
delete pending(caller, tx_name, [p,...]) :- commit_tx(caller, tx_name, [p,...]).
\end{datalog}

